Learning to Generate Explainable Stock Predictions using Self-Reflective Large Language Models

Explaining stock predictions is generally a difficult task for traditional non-generative deep learning models, where explanations are limited to visualizing the attention weights on important texts. Today, Large Language Models (LLMs) present a solution to this problem, given their known capabilities to generate human-readable explanations for their decision-making process. However, the task of stock prediction remains challenging for LLMs, as it requires the ability to weigh the varying impacts of chaotic social texts on stock prices. The problem gets progressively harder with the introduction of the explanation component, which requires LLMs to explain verbally why certain factors are more important than the others. On the other hand, to fine-tune LLMs for such a task, one would need expert-annotated samples of explanation for every stock movement in the training set, which is expensive and impractical to scale. To tackle these issues, we propose our Summarize-Explain-Predict (SEP) framework, which utilizes a self-reflective agent and Proximal Policy Optimization (PPO) to let a LLM teach itself how to generate explainable stock predictions in a fully autonomous manner. The reflective agent learns how to explain past stock movements through self-reasoning, while the PPO trainer trains the model to generate the most likely explanations from input texts. The training samples for the PPO trainer are also the responses generated during the reflective process, which eliminates the need for human annotators. Using our SEP framework, we fine-tune a LLM that can outperform both traditional deep-learning and LLM methods in prediction accuracy and Matthews correlation coefficient for the stock classification task. To justify the generalization capability of our framework, we further test it on the portfolio construction task, and demonstrate its effectiveness through various portfolio metrics.

==> D_hallucination.tex <==
% \vspace{-10px}
% \section{Hallucination Examples}\label{hallucination}
% For the summarization, explanation and reflection tasks, we evaluate two different models for generating the responses: OpenAI GPT-3.5-turbo-16k and Vicuna-13b-v1.5-16k. For the Vicuna model, we observed that the LLM sometimes produce hallucinated responses. This resulted in poorer explanation samples for fine-tuning our SEP model, which could lead to lower prediction accuracy. In this section, we provide some examples of these hallucination cases.

% \begin{figure}[!htbp]
% \vspace{-3px}
% \includegraphics[width=\columnwidth]{images/hallucination.png}
% \vspace{-20px}
% \caption{An example of a hallucinated response from Vicuna. [...] refers to truncated text, which are all repeated text.}
% \label{hallucination-eg}
% \vspace{-6px}
% \end{figure}

% \begin{figure}[!htbp]
% \vspace{-10px}
% \includegraphics[width=\columnwidth]{images/hallucination2.png}
% \vspace{-20px}
% \caption{Another example of a hallucinated response from Vicuna. [...] refers to truncated text, which are repeated text.}
% \label{hallucination-eg2}
% \vspace{-6px}
% \end{figure}
% Figures \ref{hallucination-eg} and \ref{hallucination-eg2} show some hallucinated responses. These could be due to the LLM losing track of the task context while performing its next-word generation \cite{zhang2023siren}, or including information that it was pre-trained on but which are not relevant to its current task \cite{pu2023summarization}. 









% From the above-mentioned examples, we also address the possibility of accumulative errors in our fine-tuning process. For each stage in the SEP framework, poorly generated summaries or explanations would lead to poorer responses in the next step, which will finally culminate in bad predictions. In practice, it is possible for experts to vet through the responses first before using them in the next step, which would still be an easier task than generating the responses manually. However, more work can be done to tackle this problem, in order to solve the challenge of handling the stock prediction task with LLMs, without any human-in-the-loop. 





